Differentially Private Submodular Maximization with a Knapsack Constraint

Submodular maximization subject to a knapsack constraint (SMK) is a fundamental problem in discrete optimization, with wide-ranging applications in machine learning and related fields. As these applications increasingly involve sensitive individual data, there is a growing need for high-utility algorithms that provide formal privacy guarantees. In this work, we study the SMK problem under differential privacy, considering both monotone and non-monotone objective functions. For monotone objectives, we propose a differentially private algorithm that achieves the optimal $(1-1/e)$-approximation ratio while significantly improving both additive error and query complexity over prior work. We also present a more efficient algorithm for the same setting, achieving a $1/2$-approximation. For non-monotone objectives, we introduce, to our knowledge, the first differentially private algorithm with provable guarantees, achieving a $1/4$-approximation in expectation and an additive error comparable to the best known for monotone objective functions.

==> src/macros.tex <==

\newcommand{\ron}[1]{\textbf{\small\textcolor{blue}{Ron: #1}}}

\makeatletter
\newcommand{\plabel}[1]{%
  \phantomsection%
  % Use the algorithm2e counter instead of ALC@line
  \edef\@currentlabel{\theAlgoLine}% 
  \label{#1}%
}
\makeatother
\makeatletter
% Define a "WITH" block with proper indentation logic
\newcommand{\WITH}[1]{%
  \ALC@it\algorithmicwith\ #1\ \algorithmicdo%
  \begin{ALC@g}% Starts the indentation group
}

\newcommand{\algorithmicwith}{\textbf{with}}

% Define ENDWITH to close the indentation group
\newcommand{\ENDWITH}{%
  \end{ALC@g}% Ends the indentation group
  \ALC@it\algorithmicendwith%
}

\newcommand{\algorithmicendwith}{\textbf{end with}}
\makeatother
 
\def\ba{\ensuremath{\mathbf{a}}}
\def\bi{\ensuremath{\mathbf{i}}}
\def\bj{\ensuremath{\mathbf{j}}}
\def\bk{\ensuremath{\mathbf{k}}}
\def\bo{\ensuremath{\mathbf{0}}}
\def\bs{\ensuremath{\mathbf{s}}}
\def\bt{\ensuremath{\mathbf{t}}}
\def\bv{\ensuremath{\mathbf{v}}}
\def\bw{\ensuremath{\mathbf{w}}}
\def\bx{\ensuremath{\mathbf{x}}}
\def\bz{\ensuremath{\mathbf{z}}}
\def\bI{\ensuremath{\mathbf{I}}}
\def\bP{\ensuremath{\mathbf{P}}}
\def\bT{\ensuremath{\mathbf{T}}}
\def\bZ{\ensuremath{\mathbf{Z}}}
\def\bV{\ensuremath{\mathbf{V}}}
\def\bDelta{\ensuremath{\mathbf{\Delta}}}

\def\F{\ensuremath{\mathrm{F}}}
\def\OPT{\ensuremath{\mathrm{OPT}}}
\def\bF{\ensuremath{\mathbb{F}}}
\def\bx{\ensuremath{\mathbf{x}}}
\def\H{\ensuremath{\mathsf{H}}}
\def\N{\ensuremath{\mathbb{N}}}
\def\R{\ensuremath{\mathbb{R}}}
\def\P{\ensuremath{\mathsf{P}}}
\def\Z{\ensuremath{\mathbb{Z}}}
\def\C{\ensuremath{\mathbb{C}}}

\def\Fp{\ensuremath{\mathbb{F}_p}}
\def\Fq{\ensuremath{\mathbb{F}_q}}

\def\cA{\ensuremath{\mathcal{A}}}
\def\cP{\ensuremath{\mathcal{P}}}
\def\cD{\ensuremath{\mathcal{D}}}
\def\cM{\ensuremath{\mathcal{M}}}
\def\cN{\ensuremath{\mathcal{N}}}
\def\cO{\ensuremath{\mathcal{O}}}
\def\cL{\ensuremath{\mathcal{L}}}
\def\cF{\ensuremath{\mathcal{F}}}
\def\cH{\ensuremath{\mathcal{H}}}
\def\cR{\ensuremath{\mathcal{R}}}
\def\RR{\ensuremath{\mathcal{L}}}
\def\cE{\ensuremath{\mathcal{E}}}
\def\cC{\ensuremath{\mathcal{C}}}
\def\cG{\ensuremath{\mathcal{G}}}
\def\cS{\ensuremath{\mathcal{S}}}
\def\cX{\ensuremath{\mathcal{X}}}
\def\cY{\ensuremath{\mathcal{Y}}}
\def\cZ{\ensuremath{\mathcal{Z}}}
\def\cV{\ensuremath{\mathcal{V}}}
\def\cI{\ensuremath{\mathcal{I}}}
\newcommand{\etal}{\textit{et~al.}}

\def\Exp{\mathbb{E}}
\def\Var{\mathrm{Var}}
\def\wt{{\mathrm{wt}}}

\renewcommand{\Pr}{\mathop{\bf Pr\/}}
\def\Tr{\ensuremath{\mathsf{Tr}} }
\def\Norm{\ensuremath{\mathsf{N}} }
\newcommand{\Span}[1]{\ensuremath{\mathsf{Span}\{#1\}}}


\newcommand{\set}[1]{\ensuremath{\{ #1 \}}}
\newcommand{\Set}[1]{\ensuremath{\left\{ #1 \right\}}}
\def\cube{\ensuremath{\{ 0,1 \}}}

\newcommand{\ceil}[1]{\ensuremath{\left\lceil #1 \right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor #1 \right\rfloor}}

\def\poly{{\mathrm{poly}}}
\def\polylog{{\mathrm{polylog}}}
\newcommand{\ol}[1]{\ensuremath{\overline{#1}}}
\def\dim{{\mathrm{dim}}}

\newcommand{\eps}{\varepsilon}
\newcommand{\epshat}{\hat{\varepsilon}}
%\newcommand{\eqdef}{\stackrel{\deff}{=}}

\newcommand{\lvl}[1]{\ensuremath{^{(#1)}}}
% \newcommand{\eqdef}{\stackrel{{\rm def}}{=}}
\newcommand{\eqdef}{\triangleq}

\newcommand{\zigzag}{\textcircled{z}}


%% Ron:
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\size}[1]{\left\vert#1\right\vert}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\bbmone}{\mathbbm{1}}
\newcommand{\dotp}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\probover}[2]{\underset{#1}{\Pr}\left[{#2}\right]}


\newcommand{\E}[1]{\underset{#1}{\mathbb{E}}}
\newcommand{\Max}[1]{\underset{#1}{\max}}
\newcommand{\Eover}[2]{\underset{#1}{\mathbb{E}} \left[#2\right]}
\newcommand{\suchthat}{{\;|\;}}
\newcommand{\val}{\mathsf{val}}
\newcommand{\proj}{\ensuremath{\pi}}

\newcommand{\RW}{\mathsf{RW}}
\newcommand{\Ind}{\mathsf{Ind}}
\newcommand{\VI}{\mathrm{VI}}
% \newcommand{\Ind}{\RW_J}
\newcommand{\bias}{\mathsf{bias}}
\newcommand{\maxbias}{\mathrm{maxbias}}

% \newcommand{\Lap}[1]{\mathrm{Lap}\left(#1\right)}
\newcommand{\Lap}[1]{\mathrm{Lap}\bigl(#1\bigr)}
\newcommand{\Expo}[1]{\mathrm{Exp}\bigl(#1\bigr)}
\newcommand{\Ber}[1]{\mathrm{Ber}\left(#1\right)}
\newcommand{\Geom}[1]{\mathrm{Geom}\left(#1\right)}
\newcommand{\Bin}[2]{\mathrm{Bin}\left(#1,#2\right)}
\newcommand{\Beta}[2]{\mathrm{Beta}\left(#1,#2\right)}
\newcommand{\Gumb}[1]{\mathrm{Gumbel}\left(#1\right)}
\newcommand{\Unif}[1]{\mathrm{Unif}\left(#1\right)}


\newcommand{\supp}{\mathrm{supp}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\classes}{\mathit{classes}}
\newcommand{\score}{\mathrm{Score}}
% \newcommand{\score}{\mathrm{SScore}}
\newcommand{\globscore}{\mathrm{GlScore}}
% \newcommand{\interest}{{\mathrm{Int}_p}}
\newcommand{\cover}{\mathit{cover}}
\newcommand{\hist}{{\ensuremath{h}}}
\newcommand{\cnt}{\mathit{cnt}}
% \newcommand{\suf}{{\mathrm{Suf}_p}}
% \newcommand{\diversity}{{\mathrm{Div}_p}}
\newcommand{\similarity}{\mathit{sim}}
\newcommand{\fid}{\mathit{fid}}

\newcommand{\parity}{\mathsf{Parity}}
\newcommand{\Sum}{\mathsf{Sum}}
\newcommand{\GS}{\mathsf{GS}}
\newcommand{\nbr}{{\sim}}



\newcommand{\proboverRW}[1]{\probover{(v_1,\dots,v_t)\sim\RW_G^{t}}{#1}}
\newcommand{\proboverInd}[1]{\probover{(v_1,\dots,v_t)\sim\Ind^t}{#1}}

\newcommand{\rhomin}{\rho_{\mathsf{min}}}
\newcommand{\rhomax}{\rho_{\mathsf{max}}}
\newcommand{\sigmamax}{\sigma_{\mathsf{max}}}
\newcommand{\amax}{a_{\mathsf{max}}}

\newcommand{\PParallel}[1]{\left(#1\right)^{\parallel}}
\newcommand{\Parallel}[1]{{#1}^{\parallel}}
\newcommand{\PPerp}[1]{\left(#1\right)^{\perp}}


\newcommand{\lew}{\le_{e.w}}
\newcommand{\gew}{\ge_{e.w}}

\newcommand{\LHS}{\textit{LHS}}
\newcommand{\numclust}{{\abs{C}}}
\newcommand{\numselect}{k_{select}}

\newcommand{\cemph}[1]{\textcolor{purple}{\textit{#1}}}
\newcommand{\good}[1]{\textcolor{Green}{#1}}
\newcommand{\bad}[1]{\textcolor{red}{#1}}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\def\ourframework{$\mathsf{DPClustX}$}
\def\dpnaive{DP-Naive}
\def\tabeebaseline{$\mathsf{TabEE}$}
\def\dptabee{DP-TabEE}

\def\tvd{\mathrm{TVD}}

\newcommand{\paratitle}[1]{\vspace{1mm}\noindent\textbf{{#1}.}}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\eqnote}[1]{{\text{\footnotesize $\left( #1 \right)$}}}

%%%%%%%%%%%%%%%%%%%%% Random Variables
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}
\newcommand{\Varsymb}{\mathrm{Var}}
\DeclareMathOperator*{\ExpOp}{\Esymb}
\DeclareMathOperator*{\ProbOp}{\Psymb}

\makeatletter
%}

\def\Ex#1{%
    \ProbabilityRender{\Esymb}{#1}%
}

\def\tildeEx#1{%
    \ProbabilityRender{\widetilde{\Esymb}}{#1}%
}

\def\Var#1{%
    \ProbabilityRender{\Varsymb}{#1}%
}

\def\ProbabilityRender#1#2{%fancy probability command
  \@ifnextchar\bgroup%
  {\renderwithdist{#1}{#2}}
   {\singlervrender{#1}{#2}}
}
\def\singlervrender#1#2{%
   \ensuremath{\mathchoice
       {{#1}\left[ #2 \right]}
       {{#1}[ #2 ]}
       {{#1}[ #2 ]}
       {{#1}[ #2 ]}
   }
}
\def\renderwithdist#1#2#3{%
   \@ifnextchar\bgroup
   {\superfancyrender{#1}{#2}{#3}}
   {\ensuremath{\mathchoice
      {\underset{#2}{#1}\left[ #3 \right]}
      {{#1}_{#2}[ #3 ]}
      {{#1}_{#2}[ #3 ]}
      {{#1}_{#2}[ #3 ]}
     }
   }
}
\def\superfancyrender#1#2#3#4#5{
   \ensuremath{\mathchoice
      {\underset{#1}{{#1}}\left#4 #3 \right#5}
      {{#1}_{#2}#4 #3 #5}
      {{#1}_{#2}#4 #3 #5}
      {{#1}_{#2}#4 #3 #5}
   }
}
\makeatother


\def\expop{\ExpOp}
\def\probop{\ProbOp}

\newcommand\restrict[1]{\raisebox{-.5ex}{$|$}_{#1}}

\newcommand{\conv}[1]{\mathrm{conv}\inparen{#1}}



\newcommand{\given}{\;\vert\;}
\newcommand{\rk}{r}
\newcommand{\Ot}{\tilde{O}}
\newcommand{\ExpMech}[3]{\mathtt{EM}_{#1}\!\left(#2;#3\right)}
\newcommand{\GenExpMech}[3]{\mathtt{GEM}_{#1}\!\left(#2;#3\right)}
\newcommand{\GenRNM}[3]{\mathtt{GRNM}_{#1}\!\left(#2;#3\right)}
\newcommand{\RNM}[3]{\mathtt{RNM}_{#1}\!\left(#2;#3\right)}

\newcommand{\GenExpMechT}{$\mathtt{GEM}$\xspace}
\newcommand{\GenRNMT}{$\mathtt{GRNM}$\xspace}
\newcommand{\RNMT}{$\mathtt{RNM}$\xspace}
\newcommand{\ExpMechT}{$\mathtt{EM}$\xspace}

\newcommand{\DPTwoGG}{\texttt{DP-2GG}\xspace}
\newcommand{\TwoGG}{\texttt{2GG}\xspace}
\newcommand{\DPDGP}{\texttt{DP-DG$^+$}\xspace}
\newcommand{\DGP}{\texttt{DG$^+$}\xspace}
\newcommand{\DPSDG}{\texttt{DP-SDG}\xspace}
\newcommand{\SmkRan}{\texttt{SmkRan}\xspace}
\newcommand{\Random}{\texttt{Random}\xspace}


\newcommand{\Greedy}{\mathsf{DP-Greedy}\xspace}
\newcommand{\Selection}{\mathtt{Selection}\xspace}
\newcommand{\GuessGreedy}{\mathsf{DP-$2$-Guess Greedy}\xspace}


